Classification of spin models for Yang-Baxter planar algebras

In this paper, we classify all spin models for singly-generated Yang-Baxter planar algebras in terms of certain highly regular graphs. Using Liu's classification of singly generated Yang-Baxter planar algebras, this classifies all spin models for the Jones polynomial, the Bisch-Jones planar algebras, and the Kauffman polynomial. This simplifies and clarifies Jaeger's classification of spin models for the Kauffman polynomial. In particular, we completely avoid the opaque and computationally-taxing concept of "formal self-duality"; we also explain the numerous exceptional cases in Jaeger's classification by demonstrating a new, discrete two-parameter family of spin models for the Bisch-Jones planar algebras.

==> diagrams/tikz/cupcapshaded.tex <==
\begin{tikzpicture}[baseline = -.05cm, rounded corners = 5mm, scale = .75]
\filldraw[fill = black!40!] (-.5,-.5) -- (0,.1) -- (.5,-.5);
\filldraw[fill = black!40!] (-.5,.5) -- (0,-.1) -- (.5,.5);
\end{tikzpicture}


==> diagrams/tikz/scaledundercrossing.tex <==
\begin{tikzpicture}[baseline = -.15cm, scale = .65]
\begin{knot}[clip width = 4]
	\strand (-.5,-.5) -- (.5,.5);
	\strand (-.5,.5) -- (.5,-.5);
\end{knot}
\end{tikzpicture}
